Flip-OFDM for Optical Wireless Communications

We consider two uniploar OFDM techniques for optical wireless communications: asymmetric clipped optical OFDM (ACO-OFDM) and Flip-OFDM. Both techniques can be used to compensate multipath distortion effects in optical wireless channels. However, ACO-OFDM has been widely studied in the literature, while the performance of Flip-OFDM has never been investigated. In this paper, we conduct the performance analysis of Flip-OFDM and propose additional modification to the original scheme in order to compare the performance of both techniques. Finally, it is shown by simulation that both techniques have the same performance but different hardware complexities. In particular, for slow fading channels, Flip-OFDM offers 50% saving in hardware complexity over ACO-OFDM at the receiver.

==> Makefile <==

BIBDIR=../../bibs
TMPDIR=~/tmp

# Pattern rules:
%.eps : %.tiff
	tiff2ps $< > $@

all: two-stage-adaptive-cac.pdf two-stage-adaptive-cac.ps 

# images when they are converted to PDF. Without this switch, 
# EPS graphics in the final PDF look very fuzzy, especially when viewed with 
# a projector.
two-stage-adaptive-cac.pdf: two-stage-adaptive-cac.ps
	ps2pdf -dPDFsettings=/prepress two-stage-adaptive-cac.ps

# The -G0 parameter passed to dvips is used to get around a bug 
# in GhostScript which converts the "f" character to a pound 
# sign in the final PDF.
two-stage-adaptive-cac.ps: two-stage-adaptive-cac.dvi
	dvips -t a4 -Ppdf -G0 -f <two-stage-adaptive-cac.dvi >two-stage-adaptive-cac.ps

two-stage-adaptive-cac.dvi: two-stage-adaptive-cac.tex \
			  $(BIBDIR)/cac.bib \
			  $(BIBDIR)/abbrev.bib \
			  $(BIBDIR)/crossref.bib 
	latex two-stage-adaptive-cac
	bibtex two-stage-adaptive-cac
	latex two-stage-adaptive-cac
	latex two-stage-adaptive-cac


.PHONY: spell
spell : two-stage-adaptive-cac.tex two-stage-adaptive-cac.dict
	cat two-stage-adaptive-cac.tex | ispell  -l -t -a -p two-stage-adaptive-cac.dict | sort | uniq

.PHONY: clean
clean :
	rm -f *.dvi *.log *.aux *.bbl *.blg *.toc
	rm -f *~











